Reducing Network Load via Message Utility Estimation for Decentralized Multirobot Teams

We are motivated by quantile estimation of algae concentration in lakes and how decentralized multirobot teams can effectively tackle this problem. We find that multirobot teams improve performance in this task over single robots, and communication-enabled teams further over communication-deprived teams; however, real robots are resource-constrained, and communication networks cannot support arbitrary message loads, making naive, constant information-sharing but also complex modeling and decision-making infeasible. With this in mind, we propose online, locally computable metrics for determining the utility of transmitting a given message to the other team members and a decision-theoretic approach that chooses to transmit only the most useful messages, using a decentralized and independent framework for maintaining beliefs of other teammates. We validate our approach in simulation on a real-world aquatic dataset, and we show that restricting communication via a utility estimation method based on the expected impact of a message on future teammate behavior results in a 42% decrease in network load while simultaneously decreasing quantile estimation error by 1.84%.

==> relatedwork.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%
We are inspired by the extensive literature in utility-based
communication, and our methods share similarities with previously proposed
approaches.
% talk about different problem
Work that has considered the problem
of deciding what or when to communicate is largely motivated by the same desire
to respect bandwidth limitations that real networks must face and to reduce
communication costs, like we are here.  However, the particular methods proposed
differ in how they approach the solution and in what context the problem is
situated.  Some of the varied contexts in which utility-based decisionmaking for
inter-robot communication has been investigated include months-long data
collection to be routed to a base station \cite{padhy2010utility},
non-cooperative multi-agent path finding \cite{ma2021learning}, and
those with request-reply protocols \cite{ma2021learning,zhang2019efficient}.
% talk about utility methods
In addition, some metrics used to determine utility include message category or
intrinsic data features \cite{padhy2010utility}, difference in expected reward
after incorporating a message \cite{simonetto2014distributed,
marcotte2020optimizing, unhelkar2016contact}, and the expected effect of the
message on robot actions \cite{ma2021learning, zhang2019efficient}, the latter
of two approaches we employ in this work.


% talk specifically about the two that are most similar to our paper
Here we focus on two previous works that share many similarities with our
contribution: \cite{marcotte2020optimizing} and \cite{unhelkar2016contact}.  All
include a measure of utility based on expected reward, and the teams are
decentralized such that robots can make planning decisions and calculate their
rewards independently of others. A major difference between those and ours is
that our end goal is to explore the environment in whatever way results in the
best quantile estimates, while those works define a static goal location in the
environment for the robots to reach.  We also exclusively choose to plan using a
greedy algorithm for computational efficiency and tractability, motivated by
resource-constrained systems, and do not forward-simulate the models of other
robots while \cite{marcotte2020optimizing} does and MDPs underlie the robot
planning in both. Another significant way in which our contribution varies from
these and many other previous works is that we make the more realistic
assumption of stochastic communication on top of the communication decision; in
other words, just because a robot decides to send a message does not guarantee
that that message is received by all or any of the recipients, and furthermore,
we do not assume perfect measurement sensing. 
Despite our relatively simplistic planning and modeling methods, and more
failure-prone communication assumptions, we are able to achieve significant
decrease in network loading while maintaining good task performance.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Optimizing Multi-Robot Communication under Bandwidth Constraints
Ryan J. Marcotte · Xipeng Wang · Dhanvin Mehta · Edwin Olson
2019
\begin{itemize}
    \item abstract sounds exactly like this project
    \item uses dec-mdp model with the assumption that () st. it is tractable
    \item similar: it is factored (agetns plan and evaluate their own reward independently)
    \item contribution: uses forward simulation of other agents to evaluate the message in reward space
    \item different: Goal is to reach a goal location
    \item contribution: bandit-based comb optimization algo to select observations to communicate - can select any message that fits in the bandwidth
    \item assumes perfect communication
    \item maintains belief distribuition over transition function of teammates
    \item reward consists of reward similar to how we define it (although theirs is a penalty for taking steps before a goal location), plus a communication reward (cost) that depends on the formulation (fixed, proportional to message size, and fixed-bandwidth, which is decided offline how much to allot to each agent at each timestep); they use fixed-bandwidth, we would fall under fixed (although not all-or-nothing like they define it)
\end{itemize}

ConTaCT : Deciding to Communicate during Time-Critical
Collaborative Tasks in Unknown, Deterministic Domains
Vaibhav V. Unhelkar and Julie A. Shah
2016
\begin{itemize}
    \item also dec-mdp
    \item also uses goal states
    \item assumes perfect sensing 
    \item deemphasize uncertainty to make it more tractable
    \item ego agent maintains belief about world + estimate of others' beliefs: estimate of joint state and transition function; action policy of other agents
    \item does not forward simulate
    \item agent can decide to not use information at a step; computes expected reward for all combination of keeping to itself, not using, or fully communicating, and chooses the best action (with the highest reward)
    \item disaster response motivation (first-responder), but environment is deterministic 
\end{itemize}




Distributed Time-Varying Stochastic Optimization and Utility-based Communication.
Andrea Simonetto, Leon Kester, and Geert Leus.
2014.
\begin{itemize}
    \item stochastic optimization of a discrete-time time-varying problem
    \item other nodes use pdf of neighboring nodes, which can be chosen whether or not to send to neighbors at each time step
    \item first problem is to choose eps-error-bounded decision variables to optimally solve given function
    \item second problem is to devise utility-based policy that decides to send information that guarantees accuracy wrt eps
    \item utility metrics: locally computable difference in expected utility (improvement of objective function), then decide based on bounds whether to send updated gradient function and/or updated pdf
\end{itemize}

A Utility-Based Adaptive Sensing and Multihop Communication Protocol for Wireless Sensor Networks
PARITOSH PADHY, RAJDEEP K. DASH, KIRK MARTINEZ, and NICHOLAS R. JENNINGS.
2010.
\begin{itemize}
    \item communication to a base station - not decentralized
    \item routing protocols: data-centric (depending on data sensed attributes), hierarchical, location-based
    \item use KL divergence to value a measurement (entropy?)
    \item timescale is on the order of days
    \item cost of transmission depends on value of data and power required to transmit 
\end{itemize}

Learning Selective Communication for Multi-Agent Path Finding.
Ziyuan Ma, Yudong Luo, and Jia Pan.
2022.
\begin{itemize}
    \item relevant to Action method -- "relevant and influential" neighbors. same idea, but we are cooperative, and not path finding(?)
    \item not cooperative
    \item multi-agent path finding (MAPF)
    \item decision causal communication (DCC) is proposed
    \item neighbors are determined to be relevant and influential depending on whether their presence affects the central agent
    \item distinct from other selective comms - not cooperative/same reward - each agent has its own reward; more info is needed to swap
    \item related work: [19] transmits informative messages and allows agents to request messages based on local ambiguity. 
    \item agent requests message from another if excluding the value at that agent's location results in two different hypothetical actions 
\end{itemize}

Learning Individually Inferred Communication for Multi-Agent Cooperation.
Ziluo Ding Tiejun Huang Zongqing Lu.
2020.
\begin{itemize}
    \item I2C: Individually inferred communication. Learns a prior for 1-1 comms (learned via causal inference)
    \item NN 
\end{itemize}

Efficient Communication in Multi-Agent
Reinforcement Learning via Variance Based Control.
Sai Qian Zhang, Qi Zhang, Jieyu Lin.
2019.
\begin{itemize}
    \item request-response framework
    \item Variance Based Control (VBC) - limit variance of transferred messages
    \item each agent only communicates with others when its local decision is ambiguous - measured by difference between top two largest action values
    \item each agent only replies if its feedback is informative (variance of feedback is high)
\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% new
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

There is an extensive literature in utility-based communication and our methods share similarities with previously
proposed approaches. Work that has considered the problem
of deciding what or when to communicate is largely motivated by the same desire to respect bandwidth limitations that
real networks must face and to reduce communication costs.
However, particular methods differ in how they approach
the solution and in what context the problem is situated.
Some of the varied contexts in which utility-based decision-
making for inter-robot communication has been investigated
include months-long data collection to be routed to a base
station [3], disaster response \cite{lieser2019understanding}, non-cooperative multi-agent path finding [4], and
those with request-reply protocols [4], [5].

One common approach has been to use message category, type, or intrinsic data features [3] \cite{lieser2019understanding, barcis2021information} to determine which messages are most valuable to send. These approaches typically leverage domain knowledge for the particular application.
Previous work aimed at the problem of multirobot localization has leveraged directed acyclic graphs built by forward simulating the robot team under both transmission and non-transmission of each message \cite{anderson2021communication}. 
The goal then is to reach the best estimated group localization accuracy while minimizing the cost (number of communications required in the DAG).

The expected effect of the message on robot actions has also been used to determine utility [4], [5]. 
One approach for restricting number of communications when robots are tasked with selecting goal waypoints to visit is to use a heuristic based on limiting the new path's length, and only requesting information from others if the path would be within a certain factor length of the current path \cite{best2020decentralised}.
Monte Carlo Tree Search (MCTS) has been used within a general middleware in order to make decisions on whether a message should be sent to the network or not \cite{barcis2021information}. Their approach takes into account the temporal aspect of message utility potentially changing over time, and the tree built at each decision point includes all previous and future messages in rollouts. 
However, it does not explicitly encode network constraints and assumes that robots are always within communication range of each other.


Another class of solutions propose metrics to determine utility based on the difference in expected reward after incorporating a message [6], [7], [8]. 
In \cite{velagapudi2007maintaining}, the authors proposed a utility function computed as the sum of two competing factors: maximizing utility gained by the entire team and minimizing the number of times a message is sent. 
There, the network is point-to-point, and thus at each step, a decision is made whether to forward the received message to a random recipient or to cease forwarding.
[7] and [8] also include a
measure of utility based on expected reward, and the teams
are decentralized in terms of planning and reward calculation.
A major difference between these works and ours is that our end goal is to explore the
environment in whatever way results in the best quantile
estimates, while those define a static goal location
for the robots to reach. We also exclusively choose to
plan using a greedy algorithm for computational efficiency
and tractability, motivated by resource-constrained systems,
and do not forward-simulate the models of other robots.
% while [7] does and MDPs underlie the robot planning in both. 

Significantly, we make the (more realistic) assumption
of stochastic communication on top of the communication
decision; just because a robot decides to send a message
does not guarantee reception by all or any of the recipients.
We do not assume perfect measurement sensing. Despite
our relatively simple planning and modeling methods and
more failure-prone communication assumptions, we are able
to achieve a significant decrease in network loading while
maintaining good task performance.








Information Distribution in Multi-Robot Systems: Generic, Utility-Aware Optimization Middleware.
Michał Barciś, Agata Barciś, Nikolaos Tsiogkas and Hermann Hellwagner.
2021.
% \begin{itemize}
%     \item Best 2019 Dec-MCTS -- assumes full state is sent any time communication happens; not realistic
%     \item general information distribution middleware for deciding what to send
%     \item two parts: 1) generic optimization method, 2) evaluation model for utility of information
%     \item assumes all within comms range
%     \item categorizes information into types (battery level, position, images)
%     \item temporal aspect - utilities of types change over time and are estimated over the entire (assumed known) task horizon
%     \item does not explicitly encode network constraints
% \end{itemize}
Monte Carlo Tree Search (MCTS) has been used within a general middleware in order to make decisions on whether a message should be sent to the network or not \cite{barcis2021information}. Their approach takes into account the temporal aspect of message utility potentially changing over time, and the tree built at each decision point includes all previous and future messages in rollouts. 
However, it does not explicitly encode network constraints and assumes that robots are always within communication range of each other.


Decentralised Self-Organising Maps for Multi-Robot Information Gathering.
% Graeme Best and Geoffrey A. Hollinger.
% 2020.
% \begin{itemize}
%     \item request scores from others before claiming a goal location
%     \item propose a heuristic to only request info if adding the location would result in a path not k* longer than the current path -- to avoid unnecessary comms 
% \end{itemize}
One approach for restricting number of communications when robots are tasked with selecting goal waypoints to visit is to use a heuristic based on limiting the new path's length, and only requesting information from others if the path would be within a certain factor length of the current path \cite{best2020decentralised}.

Understanding the Impact of Message Prioritization in Post-Disaster Ad Hoc Networks
% Patrick Lieser, Nils Richerzhagen, Simon Luser, Björn Richerzhagen, Ralf Steinmetz
% 2019
% \begin{itemize}
%     \item post-disaster ad-hoc network
%     \item messages have attributes (labels, categories)
%     \item adaptive prioritization is based on largest category of waiting messages 
% \end{itemize}
based on message type (like other paper further above)

% An Incentive Mechanism for Message Relaying in Unstructured Peer-to-Peer Systems 
% Cuihong Li , Bin Yu , Katia Sycara
% 2007
% \begin{itemize}
%     \item peer to peer (P2P) message relaying system that sends rewards to others for propagating messages 
%     \item rewards result (message reception?) as opposed to action that a peer needs to take 
% \end{itemize}

Communication Planning for Cooperative Terrain-Based Underwater Localization 
Jacob Anderson * and Geoffrey A. Hollinger
2021
\begin{itemize}
    \item goal is localization + reducing load
    \item simulates forward to get value of communicating at a given step
    \item builds DAG based on the forward sims to search and find min cost comms schedule
    \item assumes comms always succeed
    \item cost is path length (number of communications required) to reach the best estimated group localization accuracy which is updated in forward sims, keeping it under some threshold (accuracy is measured in uncertainty)
\end{itemize}
Another approach, aimed at the problem of multirobot localization, has leveraged directed acyclic graphs built by forward simulating the robot team under both transmission and non-transmission of each message \cite{anderson2021communication}. 
The goal then is to reach the best estimated group localization accuracy while minimizing the cost (number of communications required in the DAG).


Maintaining Shared Belief in a Large Multiagent Team 
Prasanna Velagapudi*, Oleg Prokopyev+, Katia Sycara* and Paul Scerri*
2007
\begin{itemize}
    \item point to point (not broadcast)
    \item each decides whether or not to forward to someone else
    \item three methods tested: static TTL, modifiable TTL (+/-c at each step), and utility-based
    \item does not model others in any way (so choosing who to send to is done randomly)
    \item tokenizes messages so that they are identifiable among identical measurements
    \item utility is computed as sum of two competing factors: maximizing utility gained by entire team vs minimizing number of times message is sent
    \item 10 to 5000 agents
\end{itemize}
In \cite{velagapudi2007maintaining}, the authors proposed a utility function computed as the sum of two competing factors: maximizing utility gained by the entire team and minimizing the number of times a message is sent. 
There, the network is point-to-point, and thus at each step, a decision is made whether to forward the received message to a random recipient or to cease forwarding.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{decentralized multirobot coordination algorithms}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{modeling partially-observable other agents}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{managing network load}
things I didn't do that also address a similar problem: 
- compressing data


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


An Online Utility-Based Approach for Sampling Dynamic Ocean Fields.
Angel García-Olaya, Frédéric Py, Jnaneshwar Das, and Kanna Rajan.
2012.
\begin{itemize}
    \item just one AUV, comms not relevant
    \item multiple reward fns balance between temporal and spatial scales of sampling 
    \item can incorporate science preference or evolving knowledge about feature of interest
    \item AUV directly takes water samples, the goal is from centroid or boundary of features or control samples from ambient environment
    \item objective is not field reconstruction
    \item metric 1: good spatial coverage. metric 2: each sample covers region with similar accumulated values. metric 3: like 2, but size of regions matter
\end{itemize}

%%%%%%%% old (submitted to ICRA workshop)
There is an extensive literature in utility-based
communication and our methods share similarities with previously proposed
approaches.
% talk about different problem
Work that has considered the problem
of deciding what or when to communicate is largely motivated by the same desire
to respect bandwidth limitations that real networks must face and to reduce
communication costs.  However, particular methods 
differ in how they approach the solution and in what context the problem is
situated.  Some of the varied contexts in which utility-based decision-making for
inter-robot communication has been investigated, include months-long data
collection to be routed to a base station~\cite{padhy2010utility},
non-cooperative multi-agent path finding~\cite{ma2021learning}, and
those with request-reply protocols~\cite{ma2021learning,zhang2019efficient}.
% talk about utility methods
In addition, some metrics used to determine utility include message category or
intrinsic data features~\cite{padhy2010utility}, difference in expected reward
after incorporating a message~\cite{simonetto2014distributed,
marcotte2020optimizing, unhelkar2016contact}, and the expected effect of the
message on robot actions~\cite{ma2021learning, zhang2019efficient}, the latter
of two approaches we employ in this work.

% talk specifically about the two that are most similar to our paper
We focus on two previous works that share many similarities with our
contribution:~\cite {marcotte2020optimizing} and~\cite{unhelkar2016contact}.  All
include a measure of utility based on expected reward, and the teams are
decentralized in terms of planning and reward calculation. A major difference is
that our end goal is to explore the environment in whatever way results in the
best quantile estimates, while those works define a static goal location for the robots to reach.  We also exclusively choose to plan using a
greedy algorithm for computational efficiency and tractability, motivated by
resource-constrained systems, and do not forward-simulate the models of other
robots while~\cite{marcotte2020optimizing} does and MDPs underlie the robot
planning in both. Significantly, we make the (more realistic)
assumption of stochastic communication on top of the communication decision; just because a robot decides to send a message does not guarantee
reception by all or any of the recipients. We do not assume perfect measurement sensing. 
Despite our relatively simple planning and modeling methods and more
failure-prone communication assumptions, we are able to achieve a significant
decrease in network loading while maintaining good task performance.

